Bridging the Visual Gap: Fine-Tuning Multimodal Models with Knowledge-Adapted Captions

Recent research increasingly focuses on training vision-language models (VLMs) with long, detailed image captions. However, small-scale VLMs often struggle to balance the richness of these captions with the risk of hallucinating content during fine-tuning. In this paper, we explore how well VLMs adapt to such captions. To quantify caption quality, we propose Decomposed NLI (DNLI), an evaluation framework that breaks down generated captions into individual propositions, assessing each in isolation. This fine-grained analysis reveals a critical balance between capturing descriptive details and preventing hallucinations. Our findings show that simply reducing caption complexity or employing standard data curation techniques does not effectively resolve this issue. To tackle this challenge, we introduce Knowledge Adapted (KnowAda) fine-tuning, a data-centric approach that automatically adapts training data with the model's existing knowledge and visual understanding. KnowAda minimizes hallucinations while preserving high descriptiveness. We validate this approach across several small-scale VLMs (up to 7B parameters) and dense caption datasets, demonstrating that KnowAda effectively balances hallucination reduction and descriptiveness. Our results show that KnowAda outperforms various baselines in both automatic metrics and human evaluations. We will release our code and models.

==> 025_motivation.tex <==
\section{Removing Unknown Questions In Fine-Tuning}


\moran{This part might be removed or placed in the appendix} To motivate our proposed  method, we first examine the impact of removing the unknown information in visual questions in a constrained settings. We demonstrate that removing the unknown questions improves performance, whereas the same questions, when the model have less such knowledge gaps, can be beneficial for learning. Our focus is on the straightforward and well-defined task of optical character recognition (OCR). 

We create a training and testing dataset of questions and answers from the DOCCI train and test sets by prompting Gemini to generate OCR questions about texts in the images, reaching a total of 2464 OCR questions. We then classify known and unknown questions in the training set using the definitions of known and unknown as described in Section \ref{sec:method}. We find that there are 776 unknown questions and 1688 known questions in the dataset. 

We train PaliGemma for 8 epochs over two settings -- over the entire 2464 training questions, and over the 1688 known questions only by filtering out the unknwon questions. We evaluate every epoch across all the questions in the test-set. As can be seen in \ref{fig:ocr_plot} (left), the word-error-rate (WER) is higher when training over all the questions compared to the known questions, suggesting that the unknown questions hinder learning in PaliGemma. Next, we follow the same settings for Mini-CPM-V~\cite{yao2024minicpm}, which was shown to exhibit very strong, state-of-the-art performance on OCR tasks. Note that for the subset of unknown questions, we use PaliGemma's unknwon question. As is shown in Figure \ref{fig:ocr_plot} (right), Mini-CPM efficiently learns from all the questions. 

These findings highlight two key insights: (1) training on unknown information can be detrimental to learning, and (2) Unknown information is model-specific —- what is unknown and harmful for one model may be beneficial to another. These insights motivate our \methodname{} method, which aims to generate dense captions tailored to each specific model for enhanced learning.


